Fingerprinting Multi-exit Deep Neural Network Models via Inference Time

Transforming large deep neural network (DNN) models into the multi-exit architectures can overcome the overthinking issue and distribute a large DNN model on resource-constrained scenarios (e.g. IoT frontend devices and backend servers) for inference and transmission efficiency. Nevertheless, intellectual property (IP) protection for the multi-exit models in the wild is still an unsolved challenge. Previous efforts to verify DNN model ownership mainly rely on querying the model with specific samples and checking the responses, e.g., DNN watermarking and fingerprinting. However, they are vulnerable to adversarial settings such as adversarial training and are not suitable for the IP verification for multi-exit DNN models. In this paper, we propose a novel approach to fingerprint multi-exit models via inference time rather than inference predictions. Specifically, we design an effective method to generate a set of fingerprint samples to craft the inference process with a unique and robust inference time cost as the evidence for model ownership. We conduct extensive experiments to prove the uniqueness and robustness of our method on three structures (ResNet-56, VGG-16, and MobileNet) and three datasets (CIFAR-10, CIFAR-100, and Tiny-ImageNet) under comprehensive adversarial settings.

==> old_related_work.tex <==

\subsection{Multi-exit Models}

To accelerate the inference on resource-constrained devices, one promising research direction is to build multi-exit DNN architectures, which can selectively make predictions at earlier layers~(\cite{huang2017densely}). 
The key idea is to insert multiple ICs (i.e., exit points) at different layers in a DNN model.
The sample to be analyzed will pass through each layer one by one, and each classifier attempts to make a prediction. 
If one classifier has sufficient confidence to predict this sample, i.e., the stop criteria are met, the inference task for this sample will be done at this exit point, and the predicted label will be assigned. \figurename~\ref{fig:sdn} shows the structure of a multi-exit DNN model. 
A number of works have proposed different algorithms and methods to support this feature. For instance, \cite{huang2017multi} designed the MSDNets architecture, which can provide any time predictions and avoid any loss of prediction accuracy when directly modifying existing DNN architectures. ~\cite{kaya2019shallow} proposed the Shallow-Deep Network (SDN), which can directly convert a well-trained DNN model into a multi-exit one by inserting internal classifiers. 







% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.6\linewidth]{figures/SDN1.png}
%   \caption{Building a Shallow-Deep Network (SDN)~\cite{kaya2019shallow} multi-exit model by adding multiple exit points for prediction on a typical CNN model.}
%   \label{fig:sdn}
% \end{figure}


Such multi-exit DNN architecture provides great opportunities to enable distributed inference with higher efficiency on the edge system. We can deploy the first few layers and exit points on the local edge device, and migrate the rest computation to the remote server. Hence, even a tiny edge device can be involved for the complex model serving tasks. Besides, inference of most samples can be completed within the first few samples on the edge device. Then there is no need to send the intermediate results to the remote server for further prediction with extra network latency. This is much more efficient than the traditional DNN split learning task \cite{hauswald2014hybrid,kang2017neurosurgeon,eshratifar2019jointdnn,he2019model,he2020attacking}, where every sample has to go through all the layers on the edge and server to finish the prediction. 


